On the identifiability of copulas in bivariate competing risks models

In competing risks models, the joint distribution of the event times is not identifiable even when the margins are fully known, which has been referred to as the "identifiability crisis in competing risks analysis" (Crowder, 1991). We model the dependence between the event times by an unknown copula and show that identification is actually possible within many frequently used families of copulas. The result is then extended to the case where one margin is unknown.

==> copula_known_general_margins.tex <==

\section{Known general margins}
\label{sec:known-gener-marg}

This section is devoted to the case in which the marginal
distributions of $X$ and $Y$ are still known, but not necessarily
uniform on the unit interval.  Recall that under the assumption that
$X,Y\sim U[0,1]$ (i.e. $f_X = f_Y = 1_{[0,1]}$), we have that
\[ h(z,1) = 1- \frac{\partial}{\partial x} C (x,y)\Big|_{(z,z)}\] and
analogously for $\Delta = 0$ and we could base our considerations
concerning the identifiability of $C$ on its partial derivative along
the diagonal.  In the general case,
\begin{multline*}
  \P[X\leq x, Y\leq y] = C (F_X (x), F_Y (y))
= \int_0^{F_X(x)} \int_0^{F_Y(y)} c(u,v) dudv 
\\= \int_{-\infty}^x \int_{-\infty}^y \underbrace{f_X(u) f_Y(v)
  c(F_X(u), F_Y(v))}_{=:\tc(u,v)} dudv
=  \int_{-\infty}^x \int_{-\infty}^y \tc(u,v)dudv.
\end{multline*}

Consequently,
\begin{multline*}
  \P[Z>z,\Delta = 1] = \P[Y>X>z] \\
= \int_{x=z}^\infty \int_{y=x}^\infty
  \tc(x,y) dydx = \int_{x=F_X(z)}^1 \int_{y=F_Y(z)}^1 c(x,y) dydx
\end{multline*}

 and we have for the joint density $h$ of $(Z,\Delta)$ that
 \begin{equation}\label{eq:6b}
h(z,1) = f_X(z) \int_{y=F_Y(z)}^1 c(F_X(z),y)dy=1 - \frac{\partial}{\partial x} C(F_X(x),F_Y(y))\Big|_{(z,z)}
\end{equation}
and analogously for $h(z,0)$.


The identification results under uniform margins were based on the
observation that the copulas diagonal section could be reconstructed
using the observations.  In view of~\eqref{eq:6}, instead of studying
the behaviour of the copula $C$ on the diagonal, we now need to focus
attention on what happens along the curve
$\Psi:=(F_X(t),F_Y(t))_{t=0}^\infty$. Of course, the class of symmetric
copulas, let alone of all copulas, is not identifiable in this more general
setting. The formal argument for the non-identifiability of the family
of symmetric copulas is almost the same as for the uniform margins:
Given a symmetric copula, we modify it on some area that does not
intersect with a neighbourhood of the curve
$\Psi$ (see Figure~\ref{fig:suppq} on the
right).

As in the previous section, let us therefore focus on classes of
Archimedean copulas. Under uniform margins, we have calculated the
intersection point
$(\delta^{-1}_{C_\theta}(0),\delta^{-1}_{C_\theta}(0))$ of the
copula's zero line with the diagonal of the unit square (see
Figure~\ref{fig:zero1} on the left). The
coordinate $\zeta_\theta(0) := \delta^{-1}_{C_\theta}(0)$ was
identifiable from the observations. Under the assumptions of the
Corollary~\ref{prop:critztheta}, we showed that $\zeta_\theta(0)$ was
strictly monotonic in $\theta$, thus allowing us to identify $\theta$.

We will use the same idea in the more general setting of this section:
Let $\Phi$ be a class of generators parametrised by $\Theta$. In order
for the corresponding class of copulas to be identifiable, it is
sufficient that for any two different copulas $C_\theta$ and
$C_{\theta'}$, the resulting intersection points
$\zeta^\theta=(\zeta^\theta_x, \zeta^\theta_y)$ and $\zeta^{\theta'}$
of the copulas level curves with the curve $\Psi$ be different (see
Figure~\ref{fig:zero1} on the right).  Thus, we have the following
Theorem which is analogous to Theorem~\ref{res:one-parameter}.

\begin{theo}\label{thm:general_known_margins}
  Let $\Phi:=\{\varphi_\theta \;|\;
  \theta\in\Theta\subset\R\}\subset\Omega$ be a family of generators
  and write $C_{\theta}$ for the Archimedean copula generated by
  $\varphi_{\theta}$. For $z\in[0,1]$ and a copula $C_\theta$, denote
  by $\zeta^\theta(z)=(\zeta^\theta_x(z), \zeta^\theta_y(z))$ the
  unique intersection point of the copulas level curve of level $z$
  with the curve $\Psi=(F_X(t), F_Y(t))_{t=0}^\infty$.  If for some
  $z\in(0,1)$ the point $\zeta^\theta$ is injective as
  a function from $\Theta$ to $[0,1]^2$, then the class of copulas
  generated by $\Phi$ is identifiable under the censoring model with
  known (but general) margins $F_X$ and $F_Y$. If
  the generators in $\Phi$ are bounded, the choice $z=0$ is also
  possible.
\end{theo}
\begin{proof}{Proof}{} The proof is analogous to the one of
  Theorem~\ref{res:one-parameter}. [\textbf{write a bit more here}]
\end{proof}



\begin{coro}[Identifiability of classes of nonstrict copulas]\label{coro:critztheta_general_known_margins} 
Let $$\Phi:=\{\varphi_\theta \;|\; \theta\in\Theta\subset\R\}\subset\Omega$$ be
a family of bounded generators such that $\theta\mapsto \varphi_\theta(t)/\varphi_\theta(0)$
is strictly monotonic in $\theta$ for every $t\in(0,1)$.
Then, the copulas generated by the class $\Phi$ are identifiable. % with known (but general) margins $F_X$ and $F_Y$.
\end{coro}
\begin{proof}{Proof}{}
  First note that since a constant times a generator results in the
  same Archimedean copula, we can as well consider the following class of
  generators: $\{\varphi_\theta/\varphi_\theta(0) \;|\;
  \theta\in\Theta\subset\R\}\subset\Omega$.  This means that without
  loss of generality we may assume $\varphi_\theta(0)=1$ and that
  $\phi_\theta(t)$ is strictly monotonic in $\theta$ .

  Consider the intersection point $\zeta$ of the copulas zero curve
  with the curve defined by $\Psi=(F_X(t),F_Y(t))_{t=0}^\infty$. This
  point can be identified by means of the observations
  (cf. Theorem~\ref{thm:general_known_margins}). We show below that
  for $\theta'>\theta$, the zero curve of $C_{\theta}$ lies strictly
  above the one of $C_{\theta'}$ on $(0,1)$. This implies that two
  different choices of $\theta$ always result in two different
  intersection points $\zeta$ and thus completing the proof.

  We need to prove our claim concerning the zero curves. Recall that
  the zero curve of the copula generated by $\varphi$ is given by
  $t\mapsto \varphi^{-1}(\varphi(0) - \varphi(t))$ for $t\in[0,1]$
  (see Nelsen formula (4.3.1) on page 123). Recall further that if
  $\{f_\theta\}$ is a family of monotonic bijective functions
  $f_\theta:[0,1]\to[0,1]$ such that $f_\theta(t)$ is strictly
  increasing in $\theta$ for every $t\in (0,1)$, then
  $f^{-1}_\theta(t)$ is also strictly increasing in~$\theta$ for every
  $t\in(0,1)$ (see proof of Corollary~\ref{prop:critztheta}).

Let $t\in(0,1)$. We have that

\newcommand{\ftp}{\varphi_{\theta'}}
\newcommand{\ft}{\varphi_{\theta}}

\begin{align*}
\ftp(t) &> \ft(t)  \\
\iff  \ftp(t) &> \ft(t) - \underbrace{(\ft(0) - \ftp(0))}_{=(1-1)=0}
\\
%\iff \ftp(t) - \ftp(0) &> \ft(t) -\ft(0)\\
\iff \ft(0) - \ft(t) &> \ftp(0) - \ftp(t)\\
\iff   \ft(0) - \ft(t)  &> \ftp(\ftp^{-1}(\ftp(0)-\ftp(t)))\\
\implies   \ft(0) - \ft(t)  &> \ft(\ftp^{-1}(\ftp(0)-\ftp(t)))\\
\iff \ft^{-1}(\ft(0) - \ft(t)) &< \ftp^{-1}(\ftp(0) - \ftp(t)).
\end{align*}
This completes the proof. 
\end{proof}


[\textbf{Here examples! Remark: would the same proof not also work in
  case of uniform margins which is finally only a special case ?!}]


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "copula"
%%% End: 


==> copula_resume.tex <==
Dans le cadre des mod\`eles de risques comp\'etitifs, la distribution
jointe des temps d'\'ev\'enement n'est pas identifiable m\^eme si les lois
marginales sont enti\`erement connues, ce qui a \'et\'e appel\'e la ``crise
d'identifiabilit\'e en analyse des risques comp\'etitifs''
\citep{Cro:91}. Nous mod\'elisons la d\'ependance des temps d'\'ev\'enement \`a
l'aide d'une copule inconnue et nous montrons qu'elle est identifiable
dans des nombreuses familles de copules fr\'equemment utilis\'ees. Nous g\'en\'eralisons ensuite ce
r\'esultat au cas o\`u l'une des deux lois marginales est inconnue.



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "copula"
%%% End: 


==> copula_review.tex <==

\section{Literature review}
\label{sec:literature-review}










%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "copula"
%%% End: 

